Plants Don't Walk on the Street: Common-Sense Reasoning for Reliable Semantic Segmentation

Data-driven sensor interpretation in autonomous driving can lead to highly implausible predictions as can most of the time be verified with common-sense knowledge. However, learning common knowledge only from data is hard and approaches for knowledge integration are an active research area. We propose to use a partly human-designed, partly learned set of rules to describe relations between objects of a traffic scene on a high level of abstraction. In doing so, we improve and robustify existing deep neural networks consuming low-level sensor information. We present an initial study adapting the well-established Probabilistic Soft Logic (PSL) framework to validate and improve on the problem of semantic segmentation. We describe in detail how we integrate common knowledge into the segmentation pipeline using PSL and verify our approach in a set of experiments demonstrating the increase in robustness against several severe image distortions applied to the A2D2 autonomous driving data set.

==> PSL Paper/aknowledgments.tex <==
\paragraph{Acknowledgements}
The authors want to thank for support and useful discussions Birgit Kirsch, Julia Rosenzweig, and Dorina Weichert.
\par
The work of L.A. was supported by the Fraunhofer Center for Machine Learning within the Fraunhofer Cluster for Cognitive Internet Technologies. 
The research of S.H. was partly funded by the Federal Ministry of Education and Research of Germany as part of the competence center for machine learning ML2R (01IS18038B).

==> PSL Paper/approach.tex <==
\section{Approach}
The goal of our research is to find ways in which high-level domain knowledge can improve and robustify the predictions of deep learning models in the context of autonomous driving. 
While multiple lines of research discussed in \secref{sec:related_work} make use of domain knowledge exclusively for building a model, it is our aim to combine the data-driven approach and high-level knowledge during inference.
\par
For various traffic scenes, humans can typically use common and empirical knowledge about behaviour and features of the objects to infer their type and in-scene relations, even if generalizing to unseen scenarios.
Considering different features and interrelations of objects, this human common knowledge can partially be encoded as a set of simple rules, some of which are showcased in \figref{fig:psl-motivation}. %\ma{maybe rather parts or a sub-set can be encoded. Unsure, whether all of human knowledge can be put into a ``large set of \emph{simple} rules''.}.
The way a human would reason about such a traffic scene cannot be based on hard Boolean logic, though, in which rules hold either always or never.
For example, an object having a zebra walk underneath and standing close to a traffic sign has a high probability to be a human, as depicted in \figref{fig:psl-motivation}.
But there is a chance that this could also be something else, \eg a dog or some obstacle in a construction site.
Therefore, to integrate such high-level human knowledge in the same ``uncertain'' manner into a neural network model, we need to define logical rules with relaxed truth values.
Structuring the rules upon the identification and classification of objects aligns with the task of semantic segmentation that lends itself well to finding image regions with a common semantic, which we treat as object proposals.
%\es{don't really like this sentence but currently did not come up with better phrasing the connection of our rules with sem. seg.} \ma{What are you trying to say? That building rules upon or for object classification aligns well with the task of SemSeg, as it also identifies objects (or rather regions)?}\sh{... aligns with the task of semantic segmentation that lends itself well to finding image regions with a common semantic, which we treat as object proposals.}
We selected PSL as a framework for knowledge representation for two reasons: 
First, it allows us to flexibly use soft truth values that are suitable to define both strict and loose rules, and, second, it can be fine-tuned on data, hence, distilling high-level knowledge directly via the given annotations.
\par
We first introduce PSL in \secref{sec:PSL} and briefly describe the input requirements for a PSL program.
Based on this, \secref{sec:DerivingRules} elaborates on how we define object entities and rules in our domain of interest followed by a description of the approach to combine the PSL rules with semantic segmentation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probabilistic Soft Logic
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Probabilistic Soft Logic}
\label{sec:PSL}

Probabilistic Soft Logic (PSL)~\citep{Bach2017HLMRFsPSL,kimmig2012short} is a programming framework for probabilistic reasoning in domains with relational structure. 
Typical applications of PSL are collective classification (of interlinked objects in structured data), entity resolution (finding a mapping from multiple interrelated references to the true set of underlying entities) and link prediction (predicting whether a relationship exists between two entities). 
PSL makes use of Hinge-Loss Markov Random Fields (HL-MRF), a graphical model, and applies these to structured machine learning problems. 
%Markov Random Fields are a type of graphical model and most likely comparable to a Bayesian network, but while edges in Bayesian networks are directed, thus indicating conditional probabilities, MRFs use undirected edges to describe dependencies. \sh{look up MRFs and find succinct distinction}
Graphical models define a type of loss function that represents a probability score for each possible value configuration respecting the graph-encoded dependencies among the variables. 
For HL-MRFs~\citep{Bach2013HingeLoss,Bach2017HLMRFsPSL} the continuous loss functions are defined using the hinge loss, which allows for efficient convex optimization techniques during inference.
\par
The HL-MRFs are defined using declarative rules, whose importance can be indicated by optional non-negative \textit{weights}. 
These rules are formulated using first order logic.
%As dependencies in structural domains are often repeating patterns, PSL summarizes hinge-loss functions and weights in base elements serving as a kind of placeholder. 
%A set of these structural base elements then defines the undirected graphical model, which is grounded, \ie instantiated, given input data. 
%\par
In contrast to the binary truth values \emph{true} and \emph{false} of Boolean algebra, PSL uses continuous soft truth values in the interval $[0,1]$.
% This makes it possible to incorporate similarity functions and use \textit{most probable explanation} (MPE) inference, a continuous optimization problem which can efficiently be solved via convex optimization.
%Thus, PSL constitutes HL-MRFs as conditional, probabilistic graphical models with continuous values~\citep{Bach2017HLMRFsPSL} which can efficiently be solved via convex optimization. 
%\ma{makes in the sense of ``creates'' or ``constitutes''? Isn't PSL a sub-type of HL-MRF?}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{psl-rule-example}
    \caption{PSL rules have a conjuncted body and a single literal head. \emph{Atoms} (\eg \texttt{IntersectionUnder(O1, 'r')} are the basic elements that are used for reasoning.
    An atom is a combination of \emph{predicates} (here: \texttt{IntersectionUnder$\backslash$2}) and a sequence of variables and constants equal to the predicate's arity.
    A \emph{constant} indicates a concrete element (\eg ``\texttt{ped}'' is the concrete object class pedestrian) and a \emph{variable} denotes a placeholder later to be substituted by concrete elements.
    Here, the predicate \texttt{IntersectionUnder} has an arity of two, thus, the atom consists of the variables \texttt{O1} indicating an object plus the constant ``\texttt{r}'' indicating the underground type is the road.
    The identifier \texttt{O1} will be substituted for all available objects during inference while the constant ``\texttt{r}'' will stay the same.
    The \texttt{O1} identifier is used in three atoms indicating that during inference, each object-1-variable will be substituted by the same constant (same holds for object-2-variable \texttt{O2}, respectively).
    The exponent \texttt{\^}\texttt{2} at the end of the rule indicates that the quadratic loss is chosen. This example rule can be interpreted as \emph{``if an object 1 is placed on a sidewalk and in close distance to another object 2, which is a traffic signal, there is a probability that this object 1 is a pedestrian''}.}
    \label{fig:psl-rule-example}
\end{figure*}
%Rules in PSL can either be weighted (with non-negative values) or unweighted. 
For a detailed explanation of the elements of a PSL rule, see the example depicted in \figref{fig:psl-rule-example}. 
%The example rule in Fig.~\ref{fig:psl-rule-example} can be interpreted as \emph{``if an object 1 is placed on a sidewalk and in close distance to another object 2, which is a traffic signal, there is a probability that this object 1 is a pedestrian''}.\sh{maybe put this in the figure caption?}
\par
%\ma{While it might be too late to do substantial changes I have the impression that the explanations below are more technical than needed. At the end, we require that the ``satisfaction'' of rules can be measured in a soft-Boolean way if all ``variables'' have a definite value. If that is given we can aggregate the set of all rules to a global score using indivdual weights for each rule. Given a set of (training) observations the weights can be tuned such that  the training data coincides (or approximates) the Most Probable Explanation (MPE). The resulting fixed set of weights then allows us to perform inference over incomplete observations by choosing the most probable value for open variables. (Remark: in both cases similar inference is done, first over the space of weights, after over the (discrete) space of open variables.)}
Conceptually, we require that the ``satisfaction'' of rules can be measured in a soft-Boolean way if all ``variables'' have a defined value. In this case, we can aggregate the set of all rules to a global score using individual weights for each rule. 
Given a set of ``ground truth'' observations, the weights can be fine-tuned such that the importance of each rule agrees with the ground truth observations. 
The resulting fixed set of weights then allows us to perform inference over incomplete observations by choosing the most probable value for unknown variables.

In detail, this means each atom is mapped to a soft truth value -- before inference for all known variables, and during inference for all unknown variables.% \sh{during inference? or during weight learning?}\es{Bekannte Atoms (z.B. Sensorwerte) müssen einen Wert im Intervall [0,1] haben (im zweifel darauf skaliert werden). Für Weight Learning gilt das für die GT entsprechend auch. Unbekannte werden während der Inference dann mit einem Wert in dem Intervall gemappt, der entsprechend der MPE genügt. "Ground atoms are the basic units of reasoning in PSL. Each represents an unknown or observation of interest and can take any value in [0; 1]."}
To compute the continuous truth value of the whole rule, values on atom-level are combined using the \emph{Lukasiewicz t-norm}~\citep{klir1995fuzzy} as a relaxation for the logical conjunction, disjunction, and negation.
%
Each rule's \emph{satisfaction} is calculated indicating to what degree that rule is fulfilled given the current configuration of values.
A rule is satisfied if the head is assigned at least the same truth value as the body, and a fully satisfied rule has a value of $1$.

All possible variable configurations for the rules are combined to a probability distribution, in which those that satisfy more ground rules are more probable.
% Thus, we can consider our information from the environment to be such most probable configuration and we want to construct rules that can describe it best.
%
If a weight is assigned to a rule, this indicates the importance of this rule to be satisfied in relation to the other rules and their corresponding weights. 
Rules that are unweighted induce hard constraints which require the rule to be met at all times.
During inference, the most probable value configuration for unknown predicates is found given evidence (via known predicates).
Given ground truth, the weights of rules can also be learned with maximum-likelihood estimation. 
Thus, the importance of each rule in the rule set can be learned from the data itself.
\par
Apart from these rules, a PSL program consists of a database that defines the elements of the domain of interest as well as their relations in the form of predicates. 
The database is built up from known predicates (\ie atoms that are completely observed) and unknown predicates (\ie atoms that are unobserved and must be inferred) that are part of one of the three following sets:
(i) Necessary for all known predicates is the set of \textit{observations}. These are variable combinations with an associated soft truth value in the form of actual extracted and known data for each.
(ii) Necessary for all unknown predicates is the set of \textit{targets} that is a list of all atoms (combinations of variables) that should be inferred, therefore without any associated truth values.
(iii) For weight learning a set of \textit{truths} with actual known data (likewise observations) to be used as ground truth for all unknown predicates is necessary.
Inference in PSL is done based on the first two sets, while evaluation of the inferred predicates can be done with the test set of the \textit{truths}.
% \begin{itemize}
%     \item \textit{Observations}: variable combinations with an associated soft truth value in the form of actual extracted and known data for each. Necessary for all known predicates,
%     \item \textit{Targets}: list of all atoms (combinations of variables) that should be inferred, therefore without any associated truth values. Necessary for all unknown predicates, or
%     \item \textit{Truths}: likewise observations, actual known data to be used as ground truth for all unknown predicates. This is optional for inference, where it is only used for evaluation, but necessary for weight learning.
% \end{itemize}
%\sh{weiß nicht, ob diese aufzählung dem verständnis groß hilft, wird auch nicht mehr verwendet}
%\es{besser so als Fließtext, um es nicht so stark hervorzustellen? In der nächsten Sec. wird das "Target predicate" nochmal aufgegriffen, häufiger kommt im Text der Evaluation die "observation" vor und im Anhand werden die Predicates mit Bezug zu diesen Definitionen erwähnt. Aber natürlich können wir das auch nochmal umformulieren, um die Begriffe Observation/Target/Truths nicht zu nutzen}

There are two types of rules that are supported in PSL: logical and arithmetic rules. 
We use logical rules to encode dependencies between atoms as for example depicted in the rule in \figref{fig:psl-rule-example}.
Additionally, we need to imply an arithmetic constraint to restrict the substitution for variables further.
In our setting, we want to reason about the class of an object in the scene that can only be one of three classes, constraiing the corresponding truth values to sum up to $1$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Deriving rules from domain knowledge
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deriving Rules from Domain Knowledge}
\label{sec:DerivingRules}
\par
%The overall goal of employing PSL to camera-based perception in autonomous driving is to incorporate \mac{freely available} information about the surrounding world -- organized under common knowledge logic from humans -- as additional evidence and to integrate it into the model performing inference.
The overall goal of employing PSL to camera-based perception in autonomous driving is to identify parts of common knowledge about the traffic scene that can be readily extracted and represent it in a form that facilitates integration into the model performing inference.
Based on the input requirements for a PSL program as defined above, we first need a database, \ie objects that we want to reason about as well as their relationships encoded within chosen predicates. 
Then, we define a set of rules that carries additional relational knowledge about the domain of interest that is not yet covered by the annotated data and thus can be deployed to support and validate the perception task. 
When defining an initial set of rules, one therefore has to carefully choose the objects they link up: it should be simple to both describe their behavior and to extract them from raw data.
% Deriving the rules therefore goes hand in hand with extracting objects to reason about and their description that is the restricting bound on the amount of knowledge that can be achieved.
%Deriving rules therefore goes hand in hand with extracting objects to reason about, both to some extent bounded by the available data in our setting.

% first step: describe way of defining objects
% As a first step to generate the PSL database, the objects to reason about need to be defined. 
% We chose to specify objects in a human semantic sense and therefore focus on reasoning about pedestrians, as detection of these as vulnerable road user is an important task.
Here, we choose pedestrians, traffic signs and traffic signals as our three types of objects of interest, for which we want to infer the class.
To identify these objects in a logical setting, one would need to fall back to low-level sensor interpretation.
Typically, autonomous vehicles have diverse sensors from which objects, their attributes (\eg colors, shapes) and their surroundings (\eg area underneath, background) and their relationships (\eg distance to other objects) can be derived. 
\par
For our case study, however, we solely focus on the aspect of how external knowledge can be meaningfully integrated into an existing prediction workflow. 
We therefore purposefully deploy an oracle to extract the object entities thereby neglecting additional challenges resulting from, \eg,  unreliable sensor readings and object extraction.
Our solution is to employ the connected components on ground truth segmentation masks using additional smoothing to avoid fractured objects due to occlusion.
Additionally, we emulate a depth sensor by propagating the RGB inputs to a publicly available\footnote{\url{https://github.com/nianticlabs/monodepth2}} version of MonoDepth2~\citep{godard2019digging}. 
This ``oracle sensor'' information already allows for creating a meaningful set of objects as basis for the rules.

% second step: describe way to derive rules
Subsequently, the rules describing the objects have to be defined.
To this end, we develop an initial set of rules, for which we refine the weights later on.
As we want to reason about the objects of our three selected classes, we define our target predicate \texttt{isType(Obj,Class)}.
This is used to later infer a soft truth value for each object and the possible three classes, resulting in one class being more likely than the others.
We then base the logical reasoning for an object class on the semantic features, on the surroundings of the objects, and on their relations.
Surroundings of the objects are described with the observations (known predicates) \texttt{intersectionUnder(Obj,Class)} and \texttt{intersectionBehind(Obj,Class)}.
%For example, for a traffic sign, we would assign \texttt{intersectionUnder} a high likelihood for the classes ``pedestrian walk'' or ``street''. 
For example, to infer the class of an object to be ``traffic sign'' \texttt{intersectionUnder} should have a high likelihood for the classes ``pedestrian walk'' or ``street''.
We integrate color as a semantic feature as it is especially important for traffic signs and traffic signals with the predicate \texttt{hasColor(Obj,Color).}
Rules we defined using the color predicate are for example inspired by the officially specified color combinations of common German traffic signs.
The relations between objects are specified as a distance value based on depth readings with the known predicate \texttt{distance(Obj1,Obj2)}.
The defined rules for our setup can be found in appendix~\ref{full_set_rules}.
\par
As a final step, the knowledge gained from the set of data via probabilistic rules has to be combined with the predictions from the neural network, in this case the semantic segmentation masks.
For our conceptual demonstration we follow a simplified approach integrating scores obtained from the network as prior assumptions within the rule based framework.
%
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{images/psl_approach_diagram.png}
    \caption{Overall flow of information: Oracles are serving as a source of information for objects and depth maps and also observations for weights learning; predictions produced by the neural network are combined with PSL rules via priors.}
    \label{fig:approach_diagram}
\end{figure}
%
\par
Overall, the practical approach can be described as follows (see \figref{fig:approach_diagram}):
\begin{enumerate}
    \item Identify objects to reason about and extract them from sensor data (oracle using ground truth semantic segmentation);
    \item Construct the set of rules using expert and common knowledge;
    \item Prepare the required information from lower level sensors for the rules inference (depth, colors);
    \item Learn the weights of the rules using a training set of recorded camera frames;
    \item Perform inference with the neural network and with the rules on the test set of frames for validation, possibly using network outputs as prior.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%    DEPRECATED STUFF        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probabilistic Soft Logic
% Abandoned paragraphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%In graphical models, so called potential functions $\phi$ describe which configurations for the variables are more likely. \textit{Potential functions} or \textit{potentials} therefore represent some kind of probability score for each possible value configuration w.r.t. the dependencies between the variables. For HL-MRFs \citep{Bach2013HingeLoss}, the $m$ continuous potential functions are defined using the hinge-loss as follows: \es{not sure if the detailed mathematical definition needs to be included...ideas on how to shorten this are welcome}%
%
%\begin{equation}
    %\phi_j(\mathbf{y},\mathbf{x}) = %[\textnormal{max}\{\ell_j(\mathbf{y},\mathbf{x}),0\}]^{p_j} \:,
%\end{equation}
%
%where $\ell_j$ is a linear function of $\mathbf{y,x}$, which are vectors of variables $\mathbf{y}=(y_1,...,y_n)$ and $\mathbf{x}=(x_1,...,x_{n'})$ with joint domain $\mathbf{D} = [0,1]^{n+n'}$, and with $p_j \in \{1,2\}$.
%
%For $\{\mathbf{y}$, $\mathbf{x}\}\in \tilde{\mathbf{D}}$, with $\tilde{\mathbf{D}}\subset \mathbf{D}$ satisfying a set of inequality constraints, and nonnegative weights $w_j$, the constrained hinge-loss energy function $f_w$ is defined as:
%
%\begin{equation}
%    f_w (\mathbf{y}, \mathbf{x}) = \sum_{j=1}^m w_j \phi_j (\mathbf{y}, \mathbf{x}) \: .
%\end{equation}
%
%A HL-MRF is now defined as a log-concave probability density function that is placed over random variables $\mathbf{y}$ and conditioned on the random variables $\mathbf{x}$.
%A HL-MRF $P$ is now defined as a log-concave probability density function that is placed over the inputs of $f_w$, i.e. over random variables $\mathbf{y}$ and conditioned on the random variables $\mathbf{x}$. If $(\mathbf{y}, \mathbf{x})\notin \tilde{\mathbf{D}}$ then $P(\mathbf{y}| \mathbf{x})=0$; if $(\mathbf{y}, \mathbf{x})\in \tilde{\mathbf{D}}$ then $P$ is defined as follows:
%
%\begin{equation}
%    P(\mathbf{y}| \mathbf{x}) = \frac{1}{Z(\mathbf{w}, \mathbf{x})}\exp(-f_\mathbf{w}(\mathbf{y}, \mathbf{x}))
%\end{equation}
%where $Z(\mathbf{w}, \mathbf{x})=\int_{\mathbf{y}|(\mathbf{y}, \mathbf{x})\in \mathbf{\tilde{D}}}\exp(-f_\mathbf{w}(\mathbf{y}, \mathbf{x}))\: d\mathbf{y}\:$ \citep{Bach2017HLMRFsPSL}.
%
%This makes a HL-MRF a conditional, probabilistic graphical model with continuous values \citep{Bach2017HLMRFsPSL}. 

%\texttt{5.0: undergroundType("Object1", "sidewalk")} $\wedge$ \texttt{distance("Object1", "trafficLights", "1")} %$\rightarrow$ \texttt{objectType("Object1", "pedestrian")}
%\sh{very nice, but the layout and font type should be improved}
%\emph{Atoms} (\eg \texttt{IntersectionUnder(O1, "pw", I)} are a combination of \emph{predicates} (here: \texttt{IntersectionUnder$\backslash$3}) and \emph{terms} equal to the predicate's arity (here three terms due to the predicate's arity of three: object \texttt{O1}, underground type \texttt{"pw"} (pedestrian walk) and \texttt{I} as indicator for the same image).
%A \emph{term} can either be a \emph{constant}, indicating a concrete element~\footnote{E.g. \texttt{"ped"} (pedestrian) would be a concrete object class. In opposite to variables, constants are written in quotes.}, or a \emph{variable}, denoting a placeholder~\footnote{E.g. \texttt{objectType} could be substituted by the possible classes \texttt{"ped"}, \texttt{"tr\_signal"} or \texttt{"tr\_sign"}.} to be substituted by constants from the universe of discourse. 
%For each atom $\ell$, an \emph{interpretation} $I: \ell \rightarrow [0,1]$ is a mapping to soft truth values.

%Additionally, linear equality and inequality constraints can be used to incorporate further domain knowledge and, thus, constrain the possible values of individual atoms. Interpretations on atom-level are then merged to interpretations of the body and head of the rule w.r.t. the \emph{Lukasiewicz t-norm} as relaxation for the logical conjunction, disjunction and negation.
%
% \begin{equation}
% \begin{aligned}
%     \textnormal{Disjunction}&\;\; \ell_1 \lor \ell_2 && = min(I(\ell_1)+I(\ell_2),1) \\
%     \textnormal{Conjunction}&\;\; \ell_1 \land \ell_2 && = max(0,I(\ell_1)+I(\ell_2)-1) \\
%     \textnormal{Negation}&\;\; \lnot\, \ell_1 && = 1-I(\ell_1)
% \end{aligned}
% \end{equation}
%\ie $I(r) = 1 \;\textnormal{iff.} \;I(r_{body})\leq I(r_{head})$. Therefore, a 
%
% An overall interpretation $I(r)=I(r_{body})\to I(r_{head})$ of a rule with the implication being logically equivalent to $\lnot r_{body}\lor r_{head}$ is then calculated the following : $I(r) = \textnormal{min}\{1-I(r_{body})+I(r_{head}),\;1\}$. 
% %\sh{wieso n $I: \ell \rightarrow [0,1]^n$?}\es{$^n$ war, weil ich die Definition für ein Set aus atoms $\ell=\{\ell_1,...,\ell_n\}$ genommen hatte} 
% %\ma{Is this the same $\ell$ as used above, ie a linear function of the \emph{terms}?}
% Subsequently, given an interpretation $I$, the \emph{distance to satisfaction} $d_r(I) := \textnormal{max} \{0, I(r_{body} \} -I\{r_{head}\}\}$ for each rule $r$ is calculated, where a lower value (ideally 0) indicates that the rule is not that far from being satisfied. 
%
%COMMENTS
%\ma{so, $r_\text{body}$ is a part of the rule and as such formed by a combination of atoms $\ell$ using (soft) logical operators? And, can $I$ be applied to $r$ as the rule parts are actually atoms $\ell$? Is the interpretation the same for every rule?}\es{the mapping of atoms to values between 0 and 1 is done per atom (=Interpretation of an atom). Interpretation values are known for grounded atoms of the ground truth data. Unknown interpretation values are the values that get optimized w.r.t. the distance to satisfaction of all rules and their possible interpretations using MPE. Therefore, an interpretation is not the same for every rule. Was that understandable?}
%COMMENT
%
% As an example, the rule in Fig.~\ref{fig:psl-rule-example} could have the following interpretations: \texttt{IntersectionUnder(O1,"pw",I)}$\mapsto$\texttt{0.8}, \texttt{distance(O1, O2, I)}$\mapsto$\texttt{0.7}, \texttt{isType(O2, "tr\_signal", I)}$\mapsto$\texttt{0.6} and \texttt{isType(O1, "ped", I)}$\mapsto$\texttt{0.8}. For the body of the rule this means $I(r_{body})=\textnormal{max}(0,\;0.8+0.7+0.6-1)=1.1$ and the head of the rule is simply $I(r_{head})=0.8$. Therefore, this rule has an overall satisfaction degree of $I(r)=0.7$, \ie it is satisfied to a degree of 0.7. The distance to satisfaction thus is $d_r(I) = \textnormal{max}\{0,\;1.1-0.8\}=0.3$.

% \ma{all possible $I$ means over all possible variables, the interpretations (as functions) should always be the same functions?}\es{if you would see an interpretation as a function, then yes, it is always a mapping of a (grounded) atom to a value in [0,1]. The value of course depends on the available ground truth for the atom. If no ground truth is available for this atom, value for those interpretations get optimized w.r.t. the probability density function as described above.}
%

%A set of ground rules defines a PSL program by generating a HL-MRF with the distance to satisfaction as hinge losses. 
%The probability density function $f(I)$ is defined as 
%\begin{equation}\label{eq:prob-density-func}
%    f(I) = \frac{1}{Z}\exp[-\sum_{r\in R} w_r (d_r(I))^p]
%\end{equation}
%with the rule's weight $w_r$, the continuous normalization constant $Z$ of discrete MRFs and the loss function $p\in\{1,2\}$ being either linear or quadratic. 
%, which is done by minimizing the distance to satisfaction for each rule (the sum term in equation \ref{eq:prob-density-func}). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PSL Program and PSL Rules
% Abandoned paragraphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{PSL Program and PSL Rules}
%\label{sec:PSLprogramRules}
%In the case of observations and truths, the files not only contain variable combinations but also an associated soft truth value for each atom. \sh{evtl. zusammenfassen}
%Statements only contain combinations of variables for the open predicate that have to be reasoned about. \sh{mit oben zusammenfassen}

%The soft truth values for one object relating to each class then have to sum up to 1. The according arithmetic rule would look like this: \texttt{IsType(O, +Type, I) = 1.0 .}, which means summing up the values of the predicate \texttt{IsType} for one object \texttt{O} in one image \texttt{I} to \texttt{1.0} w.r.t. the summation variable \texttt{Class}. 
%The period (\texttt{.}) at the end of this rule indicates, that this is an unweighted rule and that it always has to hold.

% There are two types of rules that are supported in PSL: logical and arithmetic rules. The first are clauses of literals that are conjuncted in the body and disjuncted in the head of the rule as depicted in the example rule in Fig.~\ref{fig:psl-rule-example}. Arithmetic rules use arithmetic operators to formulate equality or inequality for two linear combinations of summation atoms and therefore make it possible to restrict the substitution for variables further. For example, in our setting we want to reason about the type of an object in the scene that can be one of three classes. The soft truth values for one object relating to each class then have to sum up to 1. The according arithmetic rule would look like this: \texttt{IsType(O, +Type, I) = 1.0 .}, which means summing up the values of the predicate \texttt{IsType} for one object \texttt{O} ind one image \texttt{I} to \texttt{1.0} w.r.t. the summation variable \texttt{Class}. The period (\texttt{.}) at the end of this rule indicates, that this is an unweighted rule and that it always has to hold.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Deriving rules from domain knowledge
% Abandoned paragraphs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \TODO{clarify if these notes for this section are solved:}
% \begin{itemize}
%     \item focus on task of reasoning about objects, especially pedestrians: collective reasoning can provide valuable additional information to the local (independent) predictions of semantic segmentation; outlook to further work: reason across sequences of image frames to make use of temporally continuous nature of driving scenery
%     \item Basic explanation of rule construction, weights learning, predicates definition, \es{solved?}
%     \item Way to define rules and objects \sh{also, how do we define objects} we selected \es{partly solved?}
%     \item information we employ (RGB inputs, depth recognition (MonoDepth2), semantic segmentation itself), human semantic logical reasoning as source for rules
%     \item Examples of rules (and having full list in the appendix?)\sh{complete list in the appendix sounds good, but not top priority}\es{solved?}
%     \item \es{maybe argue about the different information levels that you can get from images/semantic segmentation/computer vision/sensors as a source for the rules. }
%     \begin{itemize}
%         \item Lowest information level = pixel; 
%         \item information level with higher hierarchy = connected components, shapes, colors;
%         \item then even higher level = objects, regions, distances, relationships between objects; 
%         \item highest (?) level of information = human scene understanding and human commonsense knowledge (+semantics)?
%     \end{itemize}
% \end{itemize}

% The knowledge gained from the set of data via probabilistic rules now has to be injected into the model, performing semantic segmentation  - a neural network in our case. 
% There are several approaches that allow for knowledge injection into the neural networks but in our evaluation we postprocess predictions of the network using the rules.
% meaning that we evaluate the quality of the dynamic objects recogntion via the neural network corrected by the rules predictions for the same objects introducing priors to the scores while psl inference allows to evaluate this.


%A straightforward approach to infer rules is to test all possible combinations, however, this approach does not scale.
%to let a model learn all possible PSL rules from the data itself, \ie all possible combinations of predicates, variables and constants, and evaluate the best set of these learnt rules.
%However, making this structured learning approach scalable is still a research area open for improvements \citep{getoor18structureLearningPSL, Michelioudakis2016OnlineSL}. 
% While newer methods of searching for clauses in the data are becoming more computationally efficient, this comes at the cost of search space restrictions or approximations and the need to prune the possible clauses while retaining the important ones. 




%
%The overall goal of employing probabilistic soft logic to environment learning\sh{environment learning? what is it?}\es{Linara referred to the project that was named "environmental learning with PSL". I guess we can just rephrase this to "employing PSL to camera-based perception in autonomous driving"} is to incorporate freely available information from the surrounding world and to integrate it into the model performing inference (for semantic segmentation in our case). 
%This goal is achieved best if we have a way to extract all possible information with the help of different sources of information about the environment.\sh{not sure what you want to say here? } 
%As it is usually done, autonomous vehicles have a large amount of various sensors outputs from which might be employed. 
%The challenge that arises in this setup is the necessity of an expert who can include such sensor readings into a meaningful and useful rule. \sh{why would we need an expert to make sense of multi-modal sensor inputs?}
%In our work we used only the standard set of the sensor outputs, such as RGB images and depth maps. 
%Depth maps we produced using the publicly available~\footnote{\url{https://github.com/nianticlabs/monodepth2}} version of MonoDepth2 network~\citep{godard2019digging}. 
%This sensor information already allowed for creating a meaningful set of rules.
%\sh{i am afraid i don't get the direction of this entire paragraph}
%\par
%How to create rules? The ideal approach is to automatically generate all possible rules, \ie \sh{all combinations of predicates, variables and constants}, and evaluate them - either automatically or with the help of an expert if there are only few.
%Nevertheless, that is a known hard task~\citep{buntine1996guide} \todo{not sure that this paper is exactly what we need here, check}. 
%We decided to start the work with a set of predefined rules that were constructed using just common human knowledge.

%The next challenge is to identify an appropriate semantic level on which reasoning can be done.

%To this end, we need to identify a representation which can be easily derived from raw sensor data while it is at the same time feasible and straightforward to extract useful object entities.
%Our solution in this study is to employ the connected components with smoothing (to avoid fractured objects due to occlusion) extracted from the semantic segmentation ground truth, which serves as our oracle.
%\ma{``ground truth'' instead of ``prediction'', see next sentence?}\sh{yes, likely, but i don't get the rest of the paragraph in the right order then.} 
%Using an oracle we purposefully circumvent problems that arise from relying on different input sources prone to insufficiencies, \eg lacking or poor quality predictions, and solely focus on the aspect how external knowledge (from the oracle) can be meaningfully integrated into an existing prediction workflow of some model.
%This is a limited solution.
%If the ground truth semantic segmentation is used, it cannot be applied in the real-world run.
%If the network-predicted semantic segmentation is used, poor quality (\eg in the case of an adversarial attack on the network) might preclude to extract meaningful objects or miss objects entirely.

%\ma{We could phrase this in a more positive way: Using an ``oracle device/sensor'' we purposefully circumvent problems that arise from relying on different input sources, \eg lacking or wrong predictions, and solely focus on the aspect how external knowledge (from the oracle) can be meaningfully integrated into an existing functionality/DNN workflow.}

% The knowledge gained from the set of data via probabilistic rules now has to be injected into the model, performing semantic segmentation - a neural network in our case. 
%There are several approaches that allow for knowledge injection into the neural networks~\citep{xing2020neuroplex, xu2018semantic}, but in our evaluation we simply postprocess predictions of the network using the rules predictions. \sh{how does that fit with the rest of the section?} \TODO{Does this postprocessing description still reflect the actual experiments we did?}
%Meaning that we evaluate the quality of the dynamic objects recognition via the neural network corrected by the rules predictions for the same objects - introducing priors to the scores while PSL inference allows to evaluate this.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Using PSL with Semantic Segmentation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Using PSL with Semantic Segmentation}\label{sec:PSLwSemSeg}
%\twcomment{maybe we can speak about a kind of higher level object and that semantic segmentation is a prominent source for it?}
%\sh{what are the (usual) shortcomings of semantic segmentation that we want to address by putting PSL into the mix? why is semantic segmentation a good example for using PSL? as for example in contrast to object detection? --- semantic segmentation is well-established and tried and tested, semantic segmentation represents the entire scene, relations between objects is something best modelled with PSL, hierarchy of representation (pixel vs. objects vs. entire scene)}
%\ma{for short-coming: possibly lack of necessary or logical relations?}


%Semantic segmentation is one of the most important tasks in the context of autonomous driving. \sh{semantic segmentation has already been introduced in the previous paragraph from the previous section}
%Semantic areas of an image are the basic components used later in all kinds of tasks in an autonomous vehicle \ma{soften, one could use other approaches, eg detectors. Or possibly, concertize ``semantic areas'' as entities which can be reasoned or planned about,which would be the next higher step to apply tasks such as trajectory planning. PSL sits at the interface between this high entity level and the sensor based prediction as it allows reasoning about the plausibility of the prediction in terms of entities.}. 
%The current state-of-the-art neural networks act on the pixel level and it makes it hard to introduce any logical, human-interpretable reasoning. Getting on the higher level of super-pixels or connected components helps us to connect the two worlds - specific pixel-to-class labeling and human reasoning about environment.\sh{a similar argument has been made in the previous paragraph in the previous section}
%\sh{short, i would drop this entire paragraph}




==> PSL Paper/discussion.tex <==
\section{Discussion and Conclusion}

We propose a way to reason about high level scene properties, \ie the type or class of objects, in terms of Probabilistic Soft Logic (PSL).
Taking advantage of human knowledge, we draw information from various domains, ranging from  sensor input such as color to scene properties such as the relations and distances among object.
This approach  enables us to  include additional information from data-driven model predictions, \eg as prior assumption, and improve their prediction reliability via reasoning.
Our initial evaluation in a simplified setup features a scenario from autonomous driving and indicates that the approach is viable.
Even in tests with highly adverse input augmentations it is possible to robustify the predictions of the employed semantic segmentation network.


%In this work, we propose a way to formulate, evaluate, and take advantage of human knowledge from various domains, such as knowledge about colors or relations between objects, common-sense, and scene understanding.
%This enables us to combine model predictions and logical reasoning to improve the reliability of data-driven models.


Within the PSL framework reasoning is based on rules, \ie human understandable concepts regarding the interpretation and meaning of object relations or properties.
Besides the possibility to guide the rule creation by human expert knowledge this offers strong interpretability, the set of rules could, \eg, be audited with respect to consistency.
The relevance of each rule can be adjusted individually, where the necessary weights are either deliberately chosen or learned from a training data set.
The latter case, as demonstrated in our evaluation, can serve to validate the applicability of given rules.
This places PSL in-between human designed and data driven approaches, making it an especially suited candidate to incorporate common knowledge into fundamentally data driven applications.


%\es{"learned from raw unlabeled data": can we phrase it this way? It is only the weights we are learning and there is also the oracle that is somehow labeled data, isn't it? I would also put the emphasis of this sentence more on knowledge injection/utilization and not on semantic segmentation, e.g. "In this work we proposed a way to utilize additional knowledge of different information levels, such as knowledge about colors or relations between objects, common-sense and scene understanding, to combine model predictions and logical reasoning to improve robustness. The importance of our set of rules was learned from raw unlabeled data." Something like this?}
%\ma{I think the rules are derived from human expert knowledge and optimized for the current data. Did not read far, but including human knowledge as basis is an advantage we should stress. Compare last sentence of section regarding VRUs. Additional benefits of interpretability and assurance (rules could be checked for completeness and/or consistency).}
%Our initial evaluation in a simplified setup features a scenario from autonomous driving and indicates that the approach is viable to robustify network predictions.
%using soft logic rules.
%The importance weights for this initial rule set is optimized with application-relevant data.
%We believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.
%Having obtained this optimized rule set, we show that it is possible to validate the output of trained neural networks for semantic segmentation in highly adverse scenarios.
%The fact that the human knowledge is used to formulate such a set of rules in an easily understandable syntax, plus the importance of the rules learned from the data itself, additionally provides better interpretability to the model predictions.
%The fact that PSL rules are expressed in a simple and understandable syntax and, on the other hand, weighted by given data endows the system with straightforward layer of interpretability in which the validity of certain predicates can be observed after PSL inference.

This work showcases the potential benefits such common knowledge can have for the reliability of a machine learning framework.
At this early stage we, however, neglected the cumbersome step to obtain the entities the PSL framework reasons about.
In practice this information has to be aggregated from various, most likely not fully reliable, sources, for instance stemming from additional sensors (\eg LIDAR) or alternative processing approaches.
While a probabilistic framework seems appropriate to deal with further uncertain input we restrict this demonstration to only a single ML model providing the semantic segmentation mask.
The entities and their further attributes are instead given by an oracle using the ground truth annotation.
This allows us to test the approach without the necessity to instantiate a full framework.
Another important step is the involvement of human experts for rules formulation. The presented rules are formulated with the common knowledge of the driving situations and environment, but setup specific rules, as well as the rules that are tuning a particular aspect of recognition need multiple iterations over the rules construction process.

% In our view, the main caveats that remain to be addressed in future work are high-level object selection and the principled construction of a meaningful set of the rules:
% First, in order to focus this work on the aptitude of PSL knowledge integration, we resorted to defining object entities using ground truth data. 
% Whether it will be possible to use potentialy noisy data from different sensors (\eg LIDAR) to generate object proposals of sufficient quality remains to be examined.
% Second, the rules from our experiments have been selected in a thoughtful but not systematic approach. 
% This procedure has to be investigated in order to decide if starting from and optimizing over a in some sense complete set of initial rules will result in better outcomes. 
%The rules encoding the human common understanding of the environment are the basic part of the approach.
%We decided to derive them from human knowledge instead of automatic rule learning -- this method offers a way to combine human and machine intuition, \ie, the possibility of extending automated processing steps with human expert knowledge.
%is desirable, but not quite feasible way \es{I would not put our basic contribution = rules in one sentence with us saying we did not learn them automatically. I think this way it sounds a bit too negatively?}. Thus, it requires effort of human experts \es{maybe phrase this "effort" in a more positive way?} to write down the rules describing the setup and that might help classification \es{you mean classification of the object classes?}.
%\es{we might also add the better interpretability of the human formulated rules?}

With respect to the incorporation of machine learning models we currently only use the provided prediction.
Given the probabilistic nature of both these outputs and the PSL framework the inclusion of prediction uncertainty in terms of, \eg, calibrated softmax scores could improve the reliability further.
Adding further models as discussed above would additionally require a larger set of rules.
While the used set is sufficient for demonstration purposes enlarging it to cover more attributes seems to be a straightforward way to extend our work.
Specific follow up questions could address a more systematic approach to rule building, which investigates the interplay between the set coverage, reflected by the amount and variety of rules, and its achieved performance, reflected in learned weights and task performance, more closely.
For the case of autonomous driving the incorporation of temporal consistency, requiring, \eg, that a pedestrian on two consecutive frames should not unexpectedly vanish, could add new aspects to the discussion, possibly including reasoning on the trajectories and intentions of road users.

 

% Besides the inclusion of multiple models discussed above the set or rules could be build in a more systematic way
% the work can be extended
% Second, the rules from our experiments have been selected in a thoughtful but not systematic approach. 
% This procedure has to be investigated in order to decide if starting from and optimizing over a in some sense complete set of initial rules will result in better outcomes. 

%%%%%%%%%%%%%%%%%%%%%%%%%

%There are multiple ways to follow up on the research presented in the paper.
%The most straightforward way would be to enlarge the initial set of possible predicates to cover more attributes of the objects, \eg reasoning about shapes of traffic signs or the width-height-proportion or pedestrians.
%When involving more object classes, more complex relations can be represented, \eg recognizing and treating small pedestrians as children and, thus, attributing unusual and possibly erratic behavior.
% inferring the high possibility that pedestrians are close by once a kid's ball is detected on the street.
%Focusing more on the way of knowledge integration, a more elaborate way of incorporating the knowledge from rules into the network could be introduced by taking into account uncertainty measures of the neural network predictions reflecting on what part of the prediction validation by structured knowledge is needed most.
%\es{Our initial set of rules also add the possibility to simply come up with more rules? we still had them initially (e.g. reasoning about shapes of traffic signs or the width-height-proportion or pedestrians?}
%Another direction is to widen reasoning from one frame to a sequences, using the temporally continuous nature of driving scenery.

Especially for domains such as automated driving we believe that the inclusion of human expertise into predictions is a valuable addition to safety and reliability.
Often humans are capable to infer relevant information from context.
For instance a sign indicating the potential presence of children could, by formulation of an appropriate rule, increase the likelihood that a discovered entity is inferred as child.
This inclusion of external knowledge might additionally help counterbalance the rareness of safety relevant situations, which would otherwise make it difficult to learn relevant correlations purely from data.
Deliberately fixing weights or the inclusion of specific rules as above might therefore increase the safety of vulnerable road users (VRUs) without affecting the training and optimization of the underlying machine learning models.



%Especially in domains such as automated driving we also picture the possibility of incorporating empirical knowledge.
%In this work, we defined an initial set of rules that easily could be extended to cover more empirical human knowledge.
%With only minor changes to the initial setup, our set of rules could be extended to cover more of such practical knowledge that humans gained through experience in road traffic situations.
%For example, rules reflecting the higher possibility for the appearance of pedestrians around bus stops, train stations or in traffic-calmed areas, could be based on the identification of the corresponding traffic signs.
%For example, the possibility for the appearance of pedestrians is higher around bus stops, train stations or in traffic-calmed areas.
%With slight changes to our inital setup, rules for this could be based on the identification of the corresponding traffic signs.
%Furthermore, rules could be reweighted to allow for prioritization of vulnerable road user (VRU) classes for added safety. \ma{without affecting training and optimization of underlying machine learning models.}
%\sh{ (wir haben simple regeln genommen, aber könnten auch komplexere definieren, z.b. ball heißt kind in der nähe) Rules could be modified by hand (eg chanign weights) Would allow to priorise VRU classes for added safety.} \es{anderes Beispiel mehr auf die Straßenschilder bezogen: Schild für Bushaltestelle/Bahnhof/verkehrsberuhigte Zone o.ä. bedeutet höhere Wahrscheinlichkeit, dass viele Pedestrians in der Nähe sind}
% Lastly, we believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.

==> PSL Paper/discussion_old.tex <==
\section{Discussion and Conclusion}

In this work, we propose a way to formulate, evaluate, and take advantage of human knowledge from various domains, such as knowledge about colors or relations between objects, common-sense, and scene understanding.
This enables us to combine model predictions and logical reasoning to improve the reliability of data-driven models.
\par
%\es{"learned from raw unlabeled data": can we phrase it this way? It is only the weights we are learning and there is also the oracle that is somehow labeled data, isn't it? I would also put the emphasis of this sentence more on knowledge injection/utilization and not on semantic segmentation, e.g. "In this work we proposed a way to utilize additional knowledge of different information levels, such as knowledge about colors or relations between objects, common-sense and scene understanding, to combine model predictions and logical reasoning to improve robustness. The importance of our set of rules was learned from raw unlabeled data." Something like this?}
%\ma{I think the rules are derived from human expert knowledge and optimized for the current data. Did not read far, but including human knowledge as basis is an advantage we should stress. Compare last sentence of section regarding VRUs. Additional benefits of interpretability and assurance (rules could be checked for completeness and/or consistency).}
Our initial evaluation in a simplified setup features a scenario from autonomous driving and indicates that the approach is viable to robustify network predictions.
%using soft logic rules.
The importance weights for this initial rule set is optimized with application-relevant data.
%We believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.
Having obtained this optimized rule set, we show that it is possible to validate the output of trained neural networks for semantic segmentation in highly adverse scenarios.
%The fact that the human knowledge is used to formulate such a set of rules in an easily understandable syntax, plus the importance of the rules learned from the data itself, additionally provides better interpretability to the model predictions.
The fact that PSL rules are expressed in a simple and understandable syntax and, on the other hand, weighted by given data endows the system with straightforward layer of interpretability in which the validity of certain predicates can be observed after PSL inference.
\par
In our view, the main caveats that remain to be addressed in future work are high-level object selection and the principled construction of a meaningful set of the rules:
First, in order to focus this work on the aptitude of PSL knowledge integration, we resorted to defining object entities using ground truth data. 
Whether it will be possible to use potentialy noisy data from different sensors (\eg LIDAR) to generate object proposals of sufficient quality remains to be examined.
Second, the rules from our experiments have been selected in a thoughtful but not systematic approach. 
This procedure has to be investigated in order to decide if starting from and optimizing over a in some sense complete set of initial rules will result in better outcomes. 
%The rules encoding the human common understanding of the environment are the basic part of the approach.
%We decided to derive them from human knowledge instead of automatic rule learning -- this method offers a way to combine human and machine intuition, \ie, the possibility of extending automated processing steps with human expert knowledge.
%is desirable, but not quite feasible way \es{I would not put our basic contribution = rules in one sentence with us saying we did not learn them automatically. I think this way it sounds a bit too negatively?}. Thus, it requires effort of human experts \es{maybe phrase this "effort" in a more positive way?} to write down the rules describing the setup and that might help classification \es{you mean classification of the object classes?}.
%\es{we might also add the better interpretability of the human formulated rules?}
\par
There are multiple ways to follow up on the research presented in the paper.
The most straightforward way would be to enlarge the initial set of possible predicates to cover more attributes of the objects, \eg reasoning about shapes of traffic signs or the width-height-proportion or pedestrians.
When involving more object classes, more complex relations can be represented, \eg recognizing and treating small pedestrians as children and, thus, attributing unusual and possibly erratic behavior.
% inferring the high possibility that pedestrians are close by once a kid's ball is detected on the street.
Focusing more on the way of knowledge integration, a more elaborate way of incorporating the knowledge from rules into the network could be introduced by taking into account uncertainty measures of the neural network predictions reflecting on what part of the prediction validation by structured knowledge is needed most.
%\es{Our initial set of rules also add the possibility to simply come up with more rules? we still had them initially (e.g. reasoning about shapes of traffic signs or the width-height-proportion or pedestrians?}
Another direction is to widen reasoning from one frame to a sequences, using the temporally continuous nature of driving scenery.
\par
Especially in domains such as automated driving we also picture the possibility of incorporating empirical knowledge.
%In this work, we defined an initial set of rules that easily could be extended to cover more empirical human knowledge.
With only minor changes to the initial setup, our set of rules could be extended to cover more of such practical knowledge that humans gained through experience in road traffic situations.
For example, rules reflecting the higher possibility for the appearance of pedestrians around bus stops, train stations or in traffic-calmed areas, could be based on the identification of the corresponding traffic signs.
%For example, the possibility for the appearance of pedestrians is higher around bus stops, train stations or in traffic-calmed areas.
%With slight changes to our inital setup, rules for this could be based on the identification of the corresponding traffic signs.
Furthermore, rules could be reweighted to allow for prioritization of vulnerable road user (VRU) classes for added safety.
%\sh{ (wir haben simple regeln genommen, aber könnten auch komplexere definieren, z.b. ball heißt kind in der nähe) Rules could be modified by hand (eg chanign weights) Would allow to priorise VRU classes for added safety.} \es{anderes Beispiel mehr auf die Straßenschilder bezogen: Schild für Bushaltestelle/Bahnhof/verkehrsberuhigte Zone o.ä. bedeutet höhere Wahrscheinlichkeit, dass viele Pedestrians in der Nähe sind}
% Lastly, we believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.

==> PSL Paper/evaluation.tex <==
\section{Evaluation}
The model that we selected for semantic segmentation is ERFNet~\citep{romera2017erfnet} whose lightweight encoder-decoder architecture and limited performance make it straightforward to observe the benefit of knowledge injection via PSL. 
We trained ERFNet on the A2D2 public data set \citep{geyer2020a2d2}, which features a large set of environmental scenes for cars on the road. 
The data set was separated into independent subsets (by the sequences recorded) for training and testing. 
The labels in the data set were simplified to $13$ classes via grouping. 
The network was trained using the Adam optimizer with decaying learning rate for $200$ epochs. 
The network achieved an mIoU of $0.59$ after training--in particular $0.26$ for 'Pedestrian' class and $0.63$ for 'Traffic sign' and 'Traffic signal'.

Rules selected for the evaluation first have to be ranked with weights. 
In our evaluation we obtained the weights using the learning procedure, in which the weights are assigned to the rules based on the training set with ground truth annotations. 
The observations for weight learning are extracted from the training images (predicate \texttt{hasColor}), their depth information (predicate \texttt{distance}) and the ground truth semantic segmentation (predicates \texttt{intersectionBehind} and \texttt{intersectionUnder}) using in each case the object entities from the oracle.
The full list of rules we defined along with the learned weights can be found in appendix~\ref{full_set_rules}. 
This step of weight learning serves to validate our initially proposed rules discarding those which turned out to be inadequate given the data.
In these cases, the weights assigned were in the order of $10^{-5}$. 
One such rule was for example increasing the probability of an object to be a pedestrian if it is close to an object that is a traffic sign. 

An independent test set of images is used both for evaluation of the network prediction and rule inference. 
The connected components selected as objects for soft rule-based reasoning are compared against the network predictions for the same region. 
These regions are produced using the oracle.
We refer to the ratio of correctly classified pixels as the network score for this object. 
% So, for one connected component we infer a network score for pedestrian class by counting pedestrian pixels and a network score for traffic sign class correspondingly.
% Further, the set of rules with learned weights is applied to the observations extracted from the test images, their depth information, and the network produced semantic segmentation predictions. 
Note that for weight learning we used information from the ground truth while for inference network predictions are employed. 
%\sh{are you giving all objects from the gt to the PSL framework and let it infer the object classes? is this / will this be described somewhere in approach??} \ma{think we should make the sources of the predicates (including the DNN prior) more clear, \eg is \texttt{intersectionUnder} inferred from GT or DNN prediction?}

To evaluate the robustness of the rule predictions we employed image corruptions as described by~\citet{michaelis2019dragon}. 
As the most natural we selected four, namely brightness, fog, frost and snow.
Each of them can be applied with five levels of severity, of which $1$ is the weakest (see \figref{fig:corrupt_image} for examples). 
The evaluation then follows the same route -- the network infers predictions on the corrupted images and the scores for the objects are computed. 
Likewise, rules are inferred on corrupted images and their respective predicted semantic segmentation on them. 
The oracle as further source of information is left unaffected by the applied corruptions.
\begin{figure}[th]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.46\columnwidth]{images/corruptions/20180807145028_camera_frontcenter_000012330.png}%
        \hfill
        \includegraphics[width=0.46\columnwidth]{images/corruptions/brightness_20180807145028_camera_frontcenter_000012330.png}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.46\columnwidth]{images/corruptions/fog_20180807145028_camera_frontcenter_000012330.png}%
        \hfill
        \includegraphics[width=0.46\columnwidth]{images/corruptions/frost_20180807145028_camera_frontcenter_000012330.png}
    \end{subfigure}
    \vskip\baselineskip
    \caption{Example of corruptions: original image (top left), brightness, frost and fog corruption (clockwise).}
    \label{fig:corrupt_image}
\end{figure}
The results of the predictions are depicted in \figref{fig:histograms}. 
We display the scores for the pedestrian objects, either denoting the correct or incorrect class, in the case of the original images and images corrupted with brightness. 
The histograms for the other two object classes is shown in the appendix~\ref{eval_plots}.
One can observe that the scores produced by the rules are nearly not affected--judging by the distribution of histogram peaks and the average score displayed in the legend--while network scores are very sensitive to the corruption of the data.

\begin{figure}[h]
    \centering
    \begin{subfigure}[a]{\columnwidth}
        \centering
        \includegraphics[width=0.49\columnwidth]{images/clean_run/ped_right.png}%
        \hfill
        \includegraphics[width=0.49\columnwidth]{images/clean_run/ped_wrong.png}
        \caption{Scores distribution for the objects ``pedestrians'' on the original images.}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \includegraphics[width=0.49\columnwidth]{images/brightness5_run/ped_right.png}%
        \hfill
        \includegraphics[width=0.49\columnwidth]{images/brightness5_run/ped_wrong.png}
        \caption{Scores distribution for the objects ``pedestrians'' on the corrupted (brightness, severity 5) images.}
    \end{subfigure}
    \vskip\baselineskip
    \caption{The scores of the network compared to the scores of the rules on the test dataset for pedestrian objects. It should be noted that the distribution of objects is unbalanced in the test set: the number of objects ``pedestrian'' is the smallest, followed by ``traffic signal''. The most frequent class of objects is ``traffic sign''. The network was not trained to distinguish between traffic signs or signals and we thus only report the (joined) result as ``tr\_sign'' for the wrong classes.}
    \label{fig:histograms}
\end{figure}
The final evaluation step is to combine network predictions and rules inference. 
We used the scores produced by the network as a prior for the \texttt{isType} predicate in the PSL rules.
\figref{fig:corruption_vs_score} reflects the change in the scores assigned to the objects under increasing severity of corruption. 
The scores for the objects of class ``traffic signal'' are presented here, the other classes and corruptions can be seen in the appendix~\ref{all_corr_plots}.
One can observe that the severity of the corruption affects the scores produced by a network while the inference with the rules deteriorates only slightly. 
Finally, the robustification of the network scores is also stable and shows better results than network scores on their own.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]{images/severity_corruption/frost_comparison_tr_signal.png}
    \caption{The development of average scores for the class ``traffic signal'' with  increasing severity of the ``frost'' corruption.}
    \label{fig:corruption_vs_score}
\end{figure}

==> PSL Paper/introduction.tex <==
\section{Introduction}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/psl-motivation-traffic-scene.png}
    \caption{Most humans approach the task of understanding and reasoning about traffic scenes using relations between objects. Given that all of them have been identified, common knowledge --- describing both behaviour and features, \eg relative position --- can straightforwardly be delineated in terms of simple rules. Some of the rules that we utilize in this paper are exemplified in the above figure.}
    \label{fig:psl-motivation}
\end{figure}

Deep neural networks are an integral part of autonomous driving as they achieve unmatched performance in a number of tasks, in particular image-based environment perception.
Still, they are prone to random or targeted disturbances, which renders robustness a crucial requirement for safety-critical applications. %\todo{Jan David: "please weaken, or at least say they are susceptible to various kinds of noise (without saying this prohibits safety critical application)"}
These disturbances might be of a natural source -- like overexposure, fog, snow -- or of an artificial and purposefully malicious source -- like adversarial attacks.
%This caveat concerns miniscule disturbances such as image noise, weather, or lighting conditions, as it concerns semantic changes like changes in people's clothing, architecture or vehicle models.
At the same time, wrong predictions in such tasks are most of the time blatantly obvious for human viewers that use multiple intuitive rules based on their knowledge and experience to reveal what is happening in a given scene.
Neural approaches, in their current form, aim to implicitly learn these rules from data, which makes it necessary to acquire and annotate large amounts of inputs and furthermore introduces the danger of adopting spurious correlations.
The integration of scene knowledge into the training or inference of neural networks seems a viable approach, however, this knowledge ranges from considerations of scene geometry, common knowledge, and rules of human behavior, rendering it a difficult problem \citep{vonrueden2020informed}. 
There are not only a number of competing approaches to perform the integration of knowledge itself but also multiple ways of representing the knowledge.
\par
In this paper, we study a way to represent knowledge in form of relations delineated as logic rules between identified objects in a traffic scene (see \figref{fig:psl-motivation}) and examine how these relations can be used to robustify data-driven environment perception.
To this end, we adapt the Probabilistic Soft Logic (PSL) framework~\citep{kimmig2012short} to define and learn relations between objects in the surrounding scene. 
We demonstrate the results of initial experiments aimed at quantifying its effect on the robustness of a recent small-scale semantic segmentation neural network.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%          DEPRECATED STUFF          %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \es{only some thoughts, might need rephrasing} 
% Purely data-driven ML approaches for unstructured data rely on a huge amount of training data. \sh{strange first sentence, we don't address the need for huge datasets, at least not directly}
% For example, to train deep neural networks (DNN) for the tasks of object detection or semantic segmentation, a large base of image, video data or other sensor data describing the environment in an unstructured way, is needed. 
% Especially in the area of autonomous driving, the available data sets cannot sufficiently represent all possible real-world scenarios (in particular rare cases) that might occur in everyday driving situations \TODO{(find references)}. %Using several datasets at the same time to combine their scenarios, poses other challenges as each is specialized in its particular domain  (\eg differing  architecture, traffic signs, or traffic regulations) \TODO{(add refs to some data sets)}.
%\ma{i'm not sure this first part, while true, is helpful. would psl help in ``migrating'' from one country to another or in robustness to rare situations (to which the rules might not apply in their standard form!)? Can we focus more on not-rule-modifying robustness cases as below?}
%Noise in the data, as \eg introduced by varying lighting and weather conditions, further increases complexity. 
%Another aspect is the loss of interpretability of such end-to-end, data-driven ML models. \ma{can we merge both points? the lack of interpretability makes it hard to evaluate whether or not the mL model will be robust to something or generalizes to an other case.} A way to mitigate these issues (that are not only present in the area of autonomous driving) is integrating a-priori knowledge in the learning process of deep learning models, which is an active research area \citep{vonrueden2020informed}. To tackle these limits of insufficient generalization and improve the interpretability, we therefore propose to incorporate prior knowledge in the way of human-understandable declarative rules.
%\begin{itemize}
%    \item Motivation: want to employ the massive unlabeled data in form of frames, sensor data, etc.
%    \item \es{Overall Idea here or as a separate section?} describe \textbf{overall idea}
%    \begin{itemize}
%        \item focus on how to integrate prior knowledge
%        \item oracle gives us potential objects (for the momemt we want to solve the problem of integrating knowledge via rules)
%        \item later on, we will solve the problem of substituting the oracle (maybe with sensors as additional source of information?)
%    \end{itemize}
%    \item \twcomment{Please try to abstract from PSL. The main idea is to integrate a-priori knowledge into deep learning. PSL is a way, however, we should separate the idea we have from the tools we use!}PSL as a framework for logic reasoning with soft truth values
%    \item Nice example of a rule that might be learnt \twcomment{isn't it more about fitting a model based on a-priori knowledge to data?} (e.g., person standing next to zebra most probably will start walking on it) \ma{agree with LA, rules should aid DNN. In this example rule could help prediction of dynamics (not our usecase!).}
%    \item Ways in which this can improve semantic segmentation network - adversarial robustness, noise robustness
%    \item \twcomment{I would not put to much focus on PSL. Focus on its properties an later say that we apply PSL because it is the strongest candidate satisfying the properties} \es{Ok, then maybe use the following reasons within the PSL chapter and not in the introduction}\es{possible reasons for choice of PSL: human understandable declarative rules, make us of human domain knowledge,  PSL can handle noisy sensor outputs / noisy\&incomplete data with soft truth values, fast inference}
%\end{itemize}

==> PSL Paper/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
The importance of high-level knowledge injection for image-related tasks is widely accepted~\citep{aditya2019integrating}. 
Utilizing background and common-sense knowledge about objects or regions, which goes beyond data annotations, can benefit many computer vision tasks, such as object recognition or semantic segmentation. 
Mostly due to its use in robotics and autonomous driving vehicles, semantic segmentation, as one form of low-level scene representation, is currently one of the actively developing fields in image recognition.
\par
In their survey~\citet{siam2017deep} show the development of semantic segmentation from feature-based approaches to the end-to-end deep learning networks.
Among other techniques, they point out and discuss an increase in accuracy achieved by including structural knowledge, which is abundant in the particular task of autonomous driving. %\todo{Jan David: "please remove (or strongly weaken)"}
To facilitate knowledge inclusion, according to~\citet{siam2017deep}, many researchers apply conditional random fields (CRF) additionally to deep convolutional networks for classification to improve the accuracy of the predictions.
There are also approaches that are based only on an ontology or logical reasoning for semantic segmentation. 
For example, \citet{zand2016ontology} propose to deploy Dirichlet mixture models based on super-pixel segmentation using knowledge from a fixed, user-defined ontology after which prediction is performed using conditional random fields. 
Analogously, \citet{leon2020big} use fuzzy logic to perform segmentation and \citet{dasiopoulou2005knowledge} use a high-level semantic ontology for object detection in videos.
\par
In our work, we propose to employ the PSL framework as an expressive and interpretable way to reason about the environment of the autonomous vehicle. 
To the best of our knowledge it is the first attempt to combine deep-learning-based semantic segmentation with probabilistic logical reasoning about the environment.
Nevertheless, the idea of employing knowledge via logic rules in autonomous driving tasks is not new. 
In fact, \citet{kanaujia2015markov, kardacs2013learning, kembhavi2010did} use Markov logic networks for recognizing complex events in video data.

Related work in the same area of application as ours is by \citet{souza2011probabilistic}, in which the authors use logic reasoning to support a lane detection system with high-level knowledge. 
%They employ the segmentation network output for further reasoning and controlling the movement of the vehicle (or alerting the driver).
They employ the output of their segmentation method for further reasoning and controlling the movement of the vehicle (or alerting the driver).
Similar to the PSL framework used in our work, these authors adopt Markov logic networks to employ high-level knowledge in the form of logical hard and soft rules.
However, the object-based rules are only used to classify events after recognizing objects (\eg person, car) within image frames.
In contrast, we employ soft object-based rules to robustify the prediction results of a semantic segmentation neural network for the objects in the image frames itself.
%\sh{wo ist da die knowledge injection? hört sich an, als verwenden die die ausgabe nur weiter} MA: They use a Markov Logic Network (MLN) to base a decission on the position of the vehicle and the type of road (+ few other, simple predicates). It looks (comp fig 1) like they do not merge diffrent data sources and only incorporate "traffic rules" in their downstream MLN inference based on segmentation prediction. 
Thus, our goal is to construct rules that analogously would support semantic segmentation in cases when the network itself is compromised (\eg by an image distortion) in order to prevent completely missing critical objects such as pedestrians, traffic signs or traffic signals. 
% We claim that up to our knowledge logical reasoning approaches were not used to increase robustness of semantic segmentation.
% Linara is right, sounds a little desperate, let's leave that sentence out, shall we?

==> PSL Paper/usefulCommands.tex <==
%abbreviations
%\newcommand{\ie}{i.e.,\ }
%\newcommand{\eg}{e.g.,\ }
%\newcommand{\wrt}{w.r.t.\xspace}
%\newcommand{\cf}{cf.\xspace}
%\newcommand{\etal}{et al.\xspace}

\usepackage{xcolor}
\usepackage{amsmath}

%color definitions
\definecolor{negativered}{RGB}{128, 0, 0}
\definecolor{positivegreen}{RGB}{0, 128, 0}

\definecolor{blue1}{RGB}{53, 113, 152}
\definecolor{blue2}{RGB}{65, 141, 191}
\definecolor{blue3}{RGB}{102, 164, 205}
\definecolor{blue4}{RGB}{139, 187, 218}


%comments
\newcommand{\TODO}[1]{\textcolor{red}{{\bf TODO:} #1}}
\newcommand{\TODODONE}[1]{\textcolor{green}{{\bf DONE:} #1}}


%math
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\diag}{diag}


%references
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\reftab}[1]{Tab.~\ref{#1}}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\refeqn}[1]{Eq.~\ref{#1}}


% \newcommand{\ma}[1]{\textcolor{purple}{(MA: #1)}}
% \newcommand{\mar}[1]{\textcolor{purple}{#1}}
% \newcommand{\mac}[1]{\textcolor{purple}{\sout{#1}}}
% \newcommand{\tw}[1]{\textcolor{blue}{(TW: #1)}}
% \newcommand{\sh}[1]{\textcolor{orange}{(SH: #1)}}
% \newcommand{\es}[1]{\textcolor{brown}{(ES: #1)}}
% \newcommand{\la}[1]{\textcolor{cyan}{(LA: #1)}}

==> discussion_old.tex <==
\section{Discussion and Conclusion}

In this work, we propose a way to formulate, evaluate, and take advantage of human knowledge from various domains, such as knowledge about colors or relations between objects, common-sense, and scene understanding.
This enables us to combine model predictions and logical reasoning to improve the reliability of data-driven models.
\par
%\es{"learned from raw unlabeled data": can we phrase it this way? It is only the weights we are learning and there is also the oracle that is somehow labeled data, isn't it? I would also put the emphasis of this sentence more on knowledge injection/utilization and not on semantic segmentation, e.g. "In this work we proposed a way to utilize additional knowledge of different information levels, such as knowledge about colors or relations between objects, common-sense and scene understanding, to combine model predictions and logical reasoning to improve robustness. The importance of our set of rules was learned from raw unlabeled data." Something like this?}
%\ma{I think the rules are derived from human expert knowledge and optimized for the current data. Did not read far, but including human knowledge as basis is an advantage we should stress. Compare last sentence of section regarding VRUs. Additional benefits of interpretability and assurance (rules could be checked for completeness and/or consistency).}
Our initial evaluation in a simplified setup features a scenario from autonomous driving and indicates that the approach is viable to robustify network predictions.
%using soft logic rules.
The importance weights for this initial rule set is optimized with application-relevant data.
%We believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.
Having obtained this optimized rule set, we show that it is possible to validate the output of trained neural networks for semantic segmentation in highly adverse scenarios.
%The fact that the human knowledge is used to formulate such a set of rules in an easily understandable syntax, plus the importance of the rules learned from the data itself, additionally provides better interpretability to the model predictions.
The fact that PSL rules are expressed in a simple and understandable syntax and, on the other hand, weighted by given data endows the system with straightforward layer of interpretability in which the validity of certain predicates can be observed after PSL inference.
\par
In our view, the main caveats that remain to be addressed in future work are high-level object selection and the principled construction of a meaningful set of the rules:
First, in order to focus this work on the aptitude of PSL knowledge integration, we resorted to defining object entities using ground truth data. 
Whether it will be possible to use potentialy noisy data from different sensors (\eg LIDAR) to generate object proposals of sufficient quality remains to be examined.
Second, the rules from our experiments have been selected in a thoughtful but not systematic approach. 
This procedure has to be investigated in order to decide if starting from and optimizing over a in some sense complete set of initial rules will result in better outcomes. 
%The rules encoding the human common understanding of the environment are the basic part of the approach.
%We decided to derive them from human knowledge instead of automatic rule learning -- this method offers a way to combine human and machine intuition, \ie, the possibility of extending automated processing steps with human expert knowledge.
%is desirable, but not quite feasible way \es{I would not put our basic contribution = rules in one sentence with us saying we did not learn them automatically. I think this way it sounds a bit too negatively?}. Thus, it requires effort of human experts \es{maybe phrase this "effort" in a more positive way?} to write down the rules describing the setup and that might help classification \es{you mean classification of the object classes?}.
%\es{we might also add the better interpretability of the human formulated rules?}
\par
There are multiple ways to follow up on the research presented in the paper.
The most straightforward way would be to enlarge the initial set of possible predicates to cover more attributes of the objects, \eg reasoning about shapes of traffic signs or the width-height-proportion or pedestrians.
When involving more object classes, more complex relations can be represented, \eg recognizing and treating small pedestrians as children and, thus, attributing unusual and possibly erratic behavior.
% inferring the high possibility that pedestrians are close by once a kid's ball is detected on the street.
Focusing more on the way of knowledge integration, a more elaborate way of incorporating the knowledge from rules into the network could be introduced by taking into account uncertainty measures of the neural network predictions reflecting on what part of the prediction validation by structured knowledge is needed most.
%\es{Our initial set of rules also add the possibility to simply come up with more rules? we still had them initially (e.g. reasoning about shapes of traffic signs or the width-height-proportion or pedestrians?}
Another direction is to widen reasoning from one frame to a sequences, using the temporally continuous nature of driving scenery.
\par
Especially in domains such as automated driving we also picture the possibility of incorporating empirical knowledge.
%In this work, we defined an initial set of rules that easily could be extended to cover more empirical human knowledge.
With only minor changes to the initial setup, our set of rules could be extended to cover more of such practical knowledge that humans gained through experience in road traffic situations.
For example, rules reflecting the higher possibility for the appearance of pedestrians around bus stops, train stations or in traffic-calmed areas, could be based on the identification of the corresponding traffic signs.
%For example, the possibility for the appearance of pedestrians is higher around bus stops, train stations or in traffic-calmed areas.
%With slight changes to our inital setup, rules for this could be based on the identification of the corresponding traffic signs.
Furthermore, rules could be reweighted to allow for prioritization of vulnerable road user (VRU) classes for added safety.
%\sh{ (wir haben simple regeln genommen, aber könnten auch komplexere definieren, z.b. ball heißt kind in der nähe) Rules could be modified by hand (eg chanign weights) Would allow to priorise VRU classes for added safety.} \es{anderes Beispiel mehr auf die Straßenschilder bezogen: Schild für Bushaltestelle/Bahnhof/verkehrsberuhigte Zone o.ä. bedeutet höhere Wahrscheinlichkeit, dass viele Pedestrians in der Nähe sind}
% Lastly, we believe that such a combination is beneficial not only for semantic segmentation but also for other components of autonomous car control.
